Variational Combinatorial Sequential Monte Carlo for Bayesian Phylogenetics in Hyperbolic Space

Hyperbolic space naturally encodes hierarchical structures such as phylogenies (binary trees), where inward-bending geodesics reflect paths through least common ancestors, and the exponential growth of neighborhoods mirrors the super-exponential scaling of topologies. This scaling challenge limits the efficiency of Euclidean-based approximate inference methods. Motivated by the geometric connections between trees and hyperbolic space, we develop novel hyperbolic extensions of two sequential search algorithms: Combinatorial and Nested Combinatorial Sequential Monte Carlo (\textsc{Csmc} and \textsc{Ncsmc}). Our approach introduces consistent and unbiased estimators, along with variational inference methods (\textsc{H-Vcsmc} and \textsc{H-Vncsmc}), which outperform their Euclidean counterparts. Empirical results demonstrate improved speed, scalability and performance in high-dimensional phylogenetic inference tasks.

==> Figures/circle.tex <==
% \documentclass{standalone}
% \usepackage{tikz}
% \usepackage{amsmath}

% \begin{document}

\begin{tikzpicture}[scale=3]
    % % % Axes 
    % \draw (0, -1.5) -- (0, 1.5);
    % \draw (-1.5, 0) -- (1.5, 0);
    
    % Draw the Poincaré disk (unit circle)
    \draw[thick] (0,0) circle (1cm);

    
    \draw[thick, color=blue] (.3333, 0) circle (0.6547);

    % % Origin
    % \fill (0,0) circle (1pt);
    % \node[below] at (0,0) {$O$};

    % Center - hyperbolic
    
    \node[above] at (0.8038, 0) {$\mathbf{c}$};

    % Center - Euc
    
    \node[above] at (.3333, 0) {$\mathbf{c}'$};

    % Radius - Euc
    \draw[thick, color=teal] (.3333, 0) -- (.3333, -0.6547);
    \node[left] at (.3333, -0.3274) {$r'$};

    % Radius - hyp
    % \draw[thick, color=green] (1.0239, -0.6546) arc (0:360:0.6906);
    % \draw[thick, color=green] (1.0239, -0.6546) circle (0.6906);
    \draw[thick, color=red] (.3333, -0.6547) arc (180:108.5875:0.6906);
    \node[right] at (.45, -0.3274) {$r$};

    % Left side
    
    \node[above] at (-.4, 0) {$\mathbf{x_l}$};

    
    \node[above] at (1.1, 0) {$\mathbf{x_r}$};

    \draw[fill=black, draw=black] (0.8038, 0) circle (.7pt);
    \draw[fill=black, draw=black] (.3333, 0) circle (.7pt);
    \draw[fill=black, draw=black] (-.3214, 0) circle (.7pt);
    \draw[fill=black, draw=black] (.988, 0) circle (.7pt);


\end{tikzpicture}
% \end{document}

==> Figures/twocircles.tex <==
% \documentclass{standalone}
% \usepackage{tikz}
% \usepackage{amsmath}

% \begin{document}

\begin{tikzpicture}[scale=3]
    % % % Axes 
    % \draw (0, -1.5) -- (0, 1.5);
    % \draw (-1.5, 0) -- (1.5, 0);
    
    % Draw the Poincaré disk (unit circle)
    \draw[thick] (0,0) circle (1cm);

    % Circle 1
    
    \draw[thick, color=blue] (0.3822, -0.3196) circle (0.4796);
    \node[right] at (0.6227, -0.5207) {$R$};

    % Circle 2
    
    \draw[thick, color=blue] (-0.0190,  0.3600) circle (0.6300);
    \node[left] at (-0.0439,  0.8321) {$L$};

    % Intersections
    
    % \node[right] at (0.5650, 0.1238) {$\alpha$};
    \node[right] at (0.58, 0.14) {$\alpha$};
    
    % \node[left] at (-0.0943, -0.2655) {$\tilde{\alpha}$};
    \node[left] at (-0.1, -0.35) {$\tilde{\alpha}$};

    % Geodesic
    \draw[thick, color=red] (0.6227, -0.5207) arc (224.9637:187.5004:2.3481);

    % Closest point
    
    % \node[above] at (0.1826, 0.0910) {$\mathbf{a}$};
    \node[above] at (0.2, 0.13) {$\dot{\mathbf{v}}_r^k$};
    \draw[thick, color=violet] (0.1826, 0.0910) arc (273.0392:276.7658:5.9020);
    \draw[thick, color=violet] (0.1826, 0.0910) arc (139.9687:144.3570:5.8952);

    \fill (0.6227, -0.5207) circle (.7pt);
    \fill (-0.0439,  0.8321) circle (.7pt);
    \fill (0.5650, 0.1238) circle (.7pt);
    \fill (-0.0943, -0.2655) circle (.7pt);
    \fill (0.1826, 0.0910) circle (.7pt);

\end{tikzpicture}
% \end{document}
